Number and quality of diagrams in scholarly publications is associated with number of citations

Diagrams are often used in scholarly communication. We analyse a corpus of diagrams found in scholarly computational linguistics conference proceedings (ACL 2017), and find inclusion of a system diagram to be correlated with higher numbers of citations after 3 years. Inclusion of over three diagrams in this 8-page limit conference was found to correlate with a lower citation count. Focusing on neural network system diagrams, we find a correlation between highly cited papers and "good diagramming practice" quantified by level of compliance with a set of diagramming guidelines. Two diagram classification types (one visually based, one mental model based) were not found to correlate with number of citations, but enabled quantification of heterogeneity in those dimensions. Exploring scholarly paper-writing guides, we find diagrams to be a neglected media. This study suggests that diagrams may be a useful source of quality data for predicting citations, and that "graphicacy" is a key skill for scholars with insufficient support at present.

==> approach.tex <==
Approach of this work:

Three submissions being written.

Exhibition of DIAL for rethinking ML papers - using (a more populated version of) the aidiagrams.com website and the arxiv paper.
4 page position paper on diagrammatic nanopublications, doing basic corpus analysis and (mostly already done) literature review, citing our work on R-E aswell, for rethinking ML papers. These two have a Feb 26 deadline probably. Useful intermediary for the next paper anyway:

8/16 page paper on corpus analysis targeting Diagrams conference at first. 1st April deadline.

==> tensoranalysis.tex <==
\subsection*{Another paper: Tensor representations}
%  We also have old work in support of heterogeneity, such as that in DIAL, which supports heterogeneity (Section 1.5, https://arxiv.org/pdf/1812.11142.pdf) , the R-E paper https://arxiv.org/pdf/2008.11785.pdf, and semiotic content (TWC submission, p4-7, https://www.overleaf.com/project/5bb20f1c30a2720267fe3e51)





%Vector iconography types: Circle, Square, Math, Text. Often multiple of these in the same diagram, where a different encoding is used for layers than for input or output (e.g. 189). 
Tensors, a multidimensional object describing relationships in a vector space, are a fundamental part of AI systems. In their simplest form this can be a single number, or a 2 dimensional data table. Data is manipulated in all AI systems, and visual representations of tensors (representing data) are common in diagrams of AI systems.
In natural language processing, there can be seen as two modalities for hidden layers: as a state representation or as an action. With specialisation the natural way to think about (and represent) the tensors involved here is disambiguated. The surrounding context defines this. For example, in training weights a state representation is natural, whilst in a machine translation pipeline considering hidden laters as an action is more natural.

In terms of visual encoding, it is difficult to quantify differences. Recent advances made by Richards and Engelhardt may facilitate quantitative discussion. In our domain, all systems use tensors to store data, and these tensors are commonly represented in system diagrams. 

% \subsubsection{Visual Grammar}
% Basically all of these system diagrams have different grammars, made extremely complex by the frequent use of nested figures and variety of encoding principles employed across different regions of the diagram.

%\subsection{Diagrammatic corpus analysis}
\citet{lechner2020modality} uses corpus analysis to examine the role of connecting lines in data visualisation. They examine only one connecting line in each diagram. Connecting lines are intrinsic to diagrams (diagrams being ``icons of relation"), and are also graphical objects themselves. In our analysis, we capture all tensors. 

To analyse tensors found in the corpus, we group into broad categories. The broadness of the categories is motivated by removing aspects which are likely related to the content of the system, such as whether there is repetition of objects, or whether colour is used to group. We have the following groups, based on R-E's fundamental graphical objects:
\begin{enumerate}
    \item Disks. This includes a single disk, multiple disks in a boundary, and arrays of disks.
    \item Blocks. This includes a single block, multiple blocks grouped by proximity, multiple blocks in a boundary, and arrays of blocks. This includes where a label is inside a block (i.e. a small block with an external label is categorised the same as a larger block with an internal label).
    \item Text.
    \item Mathematics (Text). Whilst this is language, as a different way of thinking about the tensor we highlight this separately.
    \item Arrows. Where an arrow is explicitly identified as a tensor (linking components is not sufficient, it needs to be signified diagrammatically or through a label or information in the caption).
    \item Unconventional. Covers other cases, such as a sphere with labels on it, graphs or numerically represented tensors and vectors.

\end{enumerate}
Further, we also record whether any instances of the tensors have a label, and if so what type (natural language, mathematical or both). The label may be grouped by proximity or contained within the graphical object. We capture all instances of tensors within the diagram, so some diagrams have multiple instances. We do not capture where an example input is used, even if the embedding step is omitted. Where different encodings exist across different diagrams, this has not been captured. This means a paper can be both high level and have a visual encoding of a tensor. There is a small degree of subjectivity in the inclusion or exclusion of some diagrams.


There are 125 system-diagram-containing papers, of which 103 include tensors. 19/125 papers were at a high level of abstraction, and did not include tensors. Three others did not include tensor representations: One mentioned this explicitly, one used visual probability distributions, and one omitted it presumably for brevity. Where we have multiple diagrams in a paper, we capture all instances used. This is because we did not want to treat subfigures differently to individually captioned figures, and because we want to explore the range of visual encodings used within a paper by the same author.

Based on our clustering method, we found 42 different combinations of tensor visual encodings. This is primarily because one diagram often uses several different visual representations for tensors. Sometimes this appears arbitrary, and sometimes it appears to signify where the embedding space differs. For example, disks are fairly commonly used to visually represent tensors within hidden layers, and mathematical notation is more common for inputs and outputs.

If one searches for differences, differences can be found between almost any pair of papers at ACL 2017 (particularly if being pedantic about size, spatial grouping or alignment).  The wide range of visual representations of tensors already demonstrates a lot of heterogeneity.


The distinction between an operation (such as an LSTM hidden node e.g. with a sigmoid activation function) and a tensor (which is the data itself) is sometimes not possible to distinguish in the diagram. From the interview study we did, it is not clear that this subtlety is understood, and is unlikely to be intentional differentiation by the author. Sometimes, it can be made explicitly component-centric by the addition of labels, use of bolding, or by context (e.g. 61b uses all of these indicators). Others (e.g. 98a, with an encoder-decoder architecture) are not clear.%, but e.g. since they use inputs in a certain visual representation, we might guess that they are considering the neural part of it in the same data-centric fashion. %(This links to philosophy paper, but is important if we're stating "visual thing X is a tensor" when actually it is an operation that they're visually representing in an identical manner to their represention of tensors elsewhere in the diagram).
In our analysis we've taken an initial impression, and the IRR gives us some confidence of the replicability of this study. Result highlights:


       
\begin{itemize}
    \item Informally, extremely few tensors were identically presented across different papers, perhaps only the blocks labelled by mathematics.
    \item The most common tensor encoding is blocks labelled by mathematics (found in 28 papers), though high level diagrams omitting any representation of tensors are also common (21 papers).
    \item Disks being used to represent tensors were identified in 42 papers, while Blocks were found in 54 papers (with overlap of 12 papers containing both). Overall, the 125 system-diagram-papers contain 38 different combinations for visually representing tensors (at the high level of ``block with label'', not whether it is an array or grouped by boundary or a solitary block, any use of colour, or where the label is). 
    \item There is a significant difference (increase) in citations between papers that include a Block labelled by Text (BLT), and those that do not (chi squared p-value $<<$0.05). This is the case even within system diagrams only. Adjusting for BLT and System Flag being correlated, there is a larger effect size. For all papers, the broad pattern is $Citations = 9.6 + 16.7*BLT + 10.9*SystemFlag$ (adjusted r-squared 0.09). Considering only system diagram papers, inclusion of a BLT is correlated with 16.7 higher average citation, almost equalling the intercept (20.5). This suggests BLT may be worth further investigation as it may be a good practice.
\end{itemize}

Limitation: Different tensor representations may be more appropriate for different applications, depending on how it is helpful to think about the system (or part of the system). For example, a stepwise process may benefit from mathematical notation, a visually-based CNN could be thought of more like pixels (blocks), and RNN-based maybe more complicated so a circle might represent some of that composite complexity (signifying that it relates to something complicated).

%extra andre thoughts: Using RE grammar to define/count the number of "steps" in the diagram, to show there is heterogeneous content being represented. Combining this with content encoding complexity explains the heterogeneous visual encoding.
